Coupling Brain-Tumor Biophysical Models and Diffeomorphic Image Registration

We present the SIBIA (Scalable Integrated Biophysics-based Image Analysis) framework for joint image registration and biophysical inversion and we apply it to analyse MR images of glioblastomas (primary brain tumors). In particular, we consider the following problem. Given the segmentation of a normal brain MRI and the segmentation of a cancer patient MRI, we wish to determine tumor growth parameters and a registration map so that if we "grow a tumor" (using our tumor model) in the normal segmented image and then register it to the patient segmented image, then the registration mismatch is as small as possible. We call this "the coupled problem" because it two-way couples the biophysical inversion and registration problems. In the image registration step we solve a large-deformation diffeomorphic registration problem parameterized by an Eulerian velocity field. In the biophysical inversion step we estimate parameters in a reaction-diffusion tumor growth model that is formulated as a partial differential equation. In this paper, our contributions are the introduction of a PDE-constrained optimization formulation of the coupled problem, the derivation of the optimality conditions, and the derivation of a Picard iterative scheme for the solution of the coupled problem. In addition, we perform several tests to experimentally assess the performance of our method on synthetic and clinical datasets. We demonstrate the convergence of the SIBIA optimization solver in different usage scenarios. We demonstrate that we can accurately solve the coupled problem in three dimensions ($256^3$ resolution) in a few minutes using 11 dual-x86 nodes. Also, we demonstrate that, with our coupled approach, we can successfully register normal MRI to tumor-bearing MRI while obtaining Dice coefficients that match those achieved when registering of normal-to-normal MRI.

==> 05-01-results_ATAV.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% TC1 ATAV-REAC: syn-tc-mov-cov #1 np=125, spacing = 1.5 sigma
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\sisetup{round-mode=places,round-precision=2}

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Purpose:} This experiment is a proof of concept. We test the numerical accuracy of our scheme, identify the inversion accuracies we can ideally expect (i.e., the errors we get if we use the forward operators to generate the observations for our coupled inversion), and study the convergence of our solver.\footnote{In general, considering real data, our forward model is---at best---a crude approximation of the actual observations. That is, first of all, we can not expect our registration algorithm to recover a bio-physically meaningful deformation between the brain anatomies of different subjects (such a model does not even exist). Second, our forward tumor model is far from being realistic (see \secref{sec:tumor} for a discussion).}

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Setup:} ATAV-REAC is based on real brain geometries, but uses a tumor grown with our forward solver in a synthetically generated patient image. We use a resolution of $N_i = 128$. We choose $\vect{p}=\vect{p}^\star$, which defines $c_A(0)=c_A^\star(0)$, grow a tumor in the tumor-free atlas, which gives $c_A^\star(1)$, choose $\vect{v}=\vect{v}^\star$, deform the atlas with the grown tumor by advecting the probability maps with the negative velocity $\vect{v}^\star$. This gives us $\vect{m}_T$ and $c_T$ (patient image with tumor). The velocity $\vect{v}^\star$ is generated by registering two tumor-free images of two different individuals ($\beta_{\vect{v}}^\star = \num{1E-4}$). The center of mass for the synthetic tumor is set to $(x^1,x^2,x^3) = 2\pi\cdot(0.285, 0.36, 0.5)$. As initial condition for the artificial tumor generation, we enable two of the Gaussians at the center of the grid of Gaussians. The same growth rates $\rho_w, \rho_g$ with scaling $\rho_f$ are used for growing the tumor and for the inversion to reconstruct the initial condition. See~\secref{s:setup} for further details on the parameters. As a baseline, we also report results for the sole registration of the healthy anatomy (i.e., neglecting the tumor forward solve to generate the data). In addition to that, we quantify the numerical error of our scheme for solving the transport equations. This is done by solving the forward problem twice, once with the original and once with the reverted (negative) velocity. The associated error is given by
\begin{equation}
\frac{\left\|c_A(1)^\star -\Rfor\left(-\vect{v}^\star,\Rfor\left(\vect{v}^\star,c_A(1)^\star\right)\right)\right\|_2}{\|c_A(1)^\star\|_2} = \num{9.372E-02}
\label{e:advection_error}
\end{equation}

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Results:} We report results for the registration of anatomy (without tumor) in \tabref{tab:reg-error-syn-tc-mov-cov}. Results for the inversion are presented in \figref{fig:mismatch_syn-ATAV-nx-128-H1SN-jacbound1E-3_betaIt-1_vdiff_c0diff} and assess the reconstruction quality (Dice and residuals) with respect to the iteration index. We also report the error between the ground truth $c_A(0)^{\star}=\Phi\vect{p}^\star$ and $\vect{v}^\star$ and the estimated iterates as well as the relative norm of the gradient of the fully coupled problem in~\eqref{eq:global_opt}.

%///////////////////////////////////////////////////////////////////////////////
\begin{table}
\caption{Results for the \textbf{analytic tumor\,/\,analytic velocity reaction-only (ATAV-REAC)} test case. We report registration-only results between healthy atlas and healthy patient. The table shows values for the relative mismatch for the geometry ($\elltwoB$) and the  associated Dice coefficient $\diceB$ as well as the relative $\ell^2$-error for the reconstruction of the velocity field $\elltwoV$ with respect to the ground truth $\vect{v}^\star$.\label{tab:reg-error-syn-tc-mov-cov}}
\centering
\begin{small}
\begin{tabular}{llll}\toprule
$\text{maxit}_R$ & \elltwoB        & $\diceB$        &  $\elltwoV$      \\\midrule
$(50,80)$        & \num{1.784e-01} & \num{9.367E-01} &  \num{3.588e-01} \\
$(10,20)$        & \num{1.675e-01} & \num{9.364E-01} &  \num{3.141e-01} \\
\bottomrule
\end{tabular}
\end{small}
\end{table}

%///////////////////////////////////////////////////////////////////////////////
\begin{figure*}[ht!]
\includegraphics[scale=.85]{figures/TC1-ATAV/{vis-all-labels-short-plain_ATAV-syn-tc}.pdf} \\
\centering
\begin{small}
\begin{tabular}{rrLlLlllll}
\toprule
iteration & $\beta_{\vect{v}}$ & $\elltwoB$         & $\diceB$           & $\elltwoT$         & $\diceT$            & $\elltwoV$         & $\delta\vect{v}$    & $\elltwoINIT$   & $\relG$           \\
\midrule
initial   &  --                & \num{1.000000e+00} & \num{7.098000e-01} & \num{1.000000e+00} & \num{0.000000e+00}  & \num{1.000000e+00} & --                  & \num{1.000e+00} & \num{1.000000e+00}\\
$1$       &  \num{1e+00}       & \num{9.371000e-01} & \num{7.270000e-01} & \num{1.000000e+00} & \num{0.000000e+00}  & \num{9.595000e-01} & --                  & \num{2.543e-01} & \num{9.976000e-01}\\
$2$       &  \num{1e-01}       & \num{6.303000e-01} & \num{8.012000e-01} & \num{2.262000e-01} & \num{8.625000e-01}  & \num{8.495000e-01} & \num{9.770000e-01}  & \num{2.047e-01} & \num{5.913000e-02}\\
$3$       &  \num{1e-02}       & \num{3.668000e-01} & \num{8.878000e-01} & \num{1.466000e-01} & \num{9.192000e-01}  & \num{6.311000e-01} & \num{9.332000e-01}  & \num{1.648e-01} & \num{3.070000e-02}\\
$4$       &  \num{1e-03}       & \num{1.706000e-01} & \num{9.396000e-01} & \num{7.910000e-02} & \num{9.661000e-01}  & \num{3.351000e-01} & \num{6.624000e-01}  & \num{1.398e-01} & \num{1.953000e-02}\\
$5$       &  \num{1e-04}       & \num{1.570000e-01} & \num{9.470000e-01} & \num{6.552000e-02} & \num{9.738000e-01}  & \num{3.594000e-01} & \num{3.649000e-01}  & \num{1.358e-01} & \num{1.322000e-02}\\
$6$       &  \num{1e-04}       & \num{1.567000e-01} & \num{9.470000e-01} & \num{6.389000e-02} & \num{9.731000e-01}  & \num{3.594000e-01} & \num{1.445000e-05}  & \num{1.330e-01} & \num{1.211000e-02}\\
$7$       &  \num{1e-04}       & \num{1.566000e-01} & \num{9.470000e-01} & \num{6.291000e-02} & \num{9.729000e-01}  & \num{3.594000e-01} & \num{1.446000e-05}  & --              & \num{1.213000e-02}\\
\bottomrule
\end{tabular}
\end{small}\\[2mm]
\caption{Results for the \textbf{analytic tumor\,/\,analytic velocity reaction-only (ATAV-REAC)} test case; ground truth: ($\rho_f=15$, $\rho_w=1$, $\rho_g=0$, $k_f=0$, $\vect{p}=\vect{p}^\star$, $\vect{v}=-\vect{v}^\star$). The figure shows probability maps for the labels of the healthy atlas brain and the patient brain with tumor generated from a tumor grown in the atlas and known atlas to patient advection velocity (see text for details; axial-slice $64$). We show the initial configuration for the problem (top row; iteration $k=1$), the final configuration after joint registration and tumor inversion (middle row; iteration $k = 7$; the atlas image probability maps are transported to the patient space), and the target patient data (reference image; bottom row). Each row contains (from left to right) the probability maps for WM, GM, CSF, and TU, the residual differences (if available) between the probability maps, and a hard segmentation based on the given probabilities for the individual tissue classes. The table on the bottom provides quantitative results for the inversion. We report the average mismatch for the probability maps for the brain tissue labels $\elltwoB$ and the tumor $\elltwoT$, the mean DICE coefficient for brain tissue $\diceB$ and tumor $\diceT$, respectively. The reconstruction quality is given in terms of convergence of $\vect{v}^k$ and $c_A^k(0)$ towards the ground truth $\vect{v}^\star$ and $c_A^\star(0)$, respectively ($\elltwoV$ and $\elltwoINIT$). We can not expect this error to go to zero for several reasons. First, we loose information when we construct the test case (zero gradients in the intensity of the image), second our numerical solver introduces errors (in particular, the solver for the transport equations).
%, and third the errors minimize the mismatch in the patient domain while our minimization works in the atlas domain.\AM{Not sure if I understand the last comment here. Why do we then not report the errors in the atlas domain? I know the reason for reporting it in the patient domain.}.
We in addition to that report the change in update in the velocity $\vect{v}$ across successive iterations $\delta\vect{v} = \|\vect{v}^k - \vect{v}^{k-1} \| / \|\vect{v}^{k-1}\|$. Finally, we also list the relative norm of the gradient for the coupled problem in~\eqref{eq:global_opt} ($\relG$).}
\label{fig:mismatch_syn-ATAV-nx-128-H1SN-jacbound1E-3_betaIt-1_vdiff_c0diff}
\end{figure*}

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Observations:} The most important observation are \bipa\item that the reconstructed data (tumor and registered anatomy) is in excellent agreement with the patient data, and \item we are able to reduce the reduced gradient~\eqref{e:reduced_gradient} by two orders of magnitude in less than 10 iterations of our Picard scheme\eipa. The Dice coefficient for the brain anatomy increases from \num{7.098000e-01} to \num{9.470000e-01}. We obtain a final Dice coefficient of \num{9.729000e-01} for the tumor.

The numerical error for the advection in~\eqref{e:advection_error} is \num{9.373e-02}. We can see in the table in~\figref{fig:mismatch_syn-ATAV-nx-128-H1SN-jacbound1E-3_betaIt-1_vdiff_c0diff} that the relative mismatch for the anatomy obtained for our iterative Picard scheme is in the order of the advection error for the forward image registration problem. We can also see that the reconstruction of $c_A(0)^\star$ and $c_A(1)^\star$ seems to be bounded by this error. In fact, due to the advection error that leads to a mismatch in this order in the atlas domain, this is the best we can expect without over-fitting the data. Similar observations can be made if we compare the results in the table in \figref{fig:mismatch_syn-ATAV-nx-128-H1SN-jacbound1E-3_betaIt-1_vdiff_c0diff} with the results obtained for the registration for healthy brains (neglecting the tumor simulations) reported in \tabref{tab:reg-error-syn-tc-mov-cov}. Hence, the quality of tumor reconstruction is comparable to the quality of pure image registration between the healthy geometries. This is an excellent result that clearly demonstrates the potential of our approach. The obtained Dice coefficient for the brain anatomy is in the order of what we see for the sole registration of healthy anatomies.\footnote{In fact, it is even slightly better. This slight increase might be a consequence of numerical inaccuracies in our scheme, discrepancies in the number of Newton-steps and Krylov iterations taken.}
Note that the mismatch between the true velocity $\vect{v}^\star$ and the recovered velocity $\vect{v}^k$ is due to the fact that image registration is an inherently ill-posed problem: the velocity can only be reconstructed exactly in image areas with non-zero gradients and if there are only non-zero intensity differences between the images to be registered in areas that do correspond to one another\footnote{As in any formulation based on an $L^2$-distance functional, it is the mismatch between the reference and template image and the gradient of the deformed template image that drive the optimization (see \eqref{opt_grad_R_solo}).}. In addition, we ask for the reconstruction of a vector field from scalar data.

We can furthermore see that we can significantly reduce the norm of the reduced gradient~\eqref{e:reduced_gradient} to  \num{1.213000e-02}. We can also see that once we have reached the target regularization parameter $\beta_{\vect{v}} = \num{1E-4}$ we do not make any more progress. The update for the velocity tends to zero, the changes in the reduced gradient are small and the error measures (residual and Dice) do no longer change significantly.

\ipoint{Conclusion:} We conclude that our Picard scheme is efficient and converges to a valid (local) minimum in the search space (we reduce the relative global gradient, the distance measure, and significantly increase the Dice coefficient). We attain an excellent agreement between the data (patient tumor and geometry) and the predicted state (transported atlas geometry and predicted tumor) with a final Dice coefficient of \num{9.470000e-01} and \num{9.729000e-01} for the labels of the anatomy and tumor, respectively.


==> 05-02-results_ATAV-DIF.tex <==
%///////////////////////////////////////////////////////////////////////////////
\ipoint{Purpose:} With this test case, we test the sensitivity of our approach with respect to pertubations in the model and model parameters.

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Setup:} The overall setup for this problem is exactly the same as used for the ATAV-REAC case in the previous section. The only differences are:
%\begin{itemize}
\begin{inparaitem}
\item We use the full model in \secref{sec:tumor}, which includes the diffusion operator to grow the tumor. %and in the Picard iterations.
\item For the inversion in the Picard iterations, we use values for the reaction and diffusion coefficients that are either the same or differ from those used for the generation of the synthetic test problem.
\end{inparaitem}
%\end{itemize}

In particular, we grow the tumor in the atlas using the growth parameters $\rho_f =10, \rho_w=1, \rho_g = 0, k_f=\num{1.0E-2}, k_w=1$ and $k_g=0$. Within the Picard iterations for the inversion, we use the 'correct' (used for growing the tumor) as well as 'wrong' reaction parameters $\rho_f \in \{5, 15\}$. We set $k_f=0$ to test if we can still reconstruct the tumor with a reaction-only model. All remaining parameters are as identified in the former sections.

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Results:} We report quantitative results for the inversion in \tabref{tab:ATAV-nonzero-diffusion} and qualitative results can be found in the supplementary material in \figref{fig:ATAV-nonzero-diffusion}. We use the same measures as we have used in the former experiments (reconstruction errors based on the Dice coefficient and the residuals for the tumor and the anatomy, and the relative reduction of the reduced gradient). We also list the runtime for the Picard scheme per iteration and the percentage spent in each individual solver (tumor and registration), respectively. Note that tumor and registration runtimes do not add up to 100\% as further parts of the code such as calculation of the reduced gradient and steering of the Picard iteration are not included in the measurements.

% %///////////////////////////////////////////////////////////////////////////////
% \begin{figure}
% \centering
% \includegraphics[width=0.48\textwidth]{figures/TC1-ATAV-DIF/rho-10/vis-ax-cor-sag-its_ATAV-syn-tc-diffusion-rho10.pdf}
% \caption{\todo{SUPPLEMENTARY MATERIAL?}Tumor and brain labels (obtained by thresholding probability maps) for the \textbf{analytic tumor with analythic velocity with non-zero diffusion (ATAV-DIF)} test case; ground truth: ($\rho_f=10$, $\rho_w=1$, $\rho_g=0$, $k_f=\num{1.0E-2}$, $k_w=1$, $k_g=0$, $\vect{p}=\vect{p}^\star$, $\vect{v}=-\vect{v}^\star$). We show results for the inversion (velocity and initial condition) if we use the true (`'correct`') tumor parameters used to generate the test case (i.e., $\rho_f=10$ and $k_f=\num{1.0E-2}$). The top row shows the initial label maps for the atlas image. The middle row shows the label maps for the atlas image after registration (transported to the patient space) and the bottom row shows the label maps for the patient data. We can see that the results are qualitatively in excellent agreement. This is confirmed by the values for the mismatch and Dice coefficients for the labels and probability maps for the individual tissue classes reported in \tabref{tab:ATAV-nonzero-diffusion}.}
% \label{fig:ATAV-nonzero-diffusion}
% \end{figure}

%///////////////////////////////////////////////////////////////////////////////
\begin{table*}
\caption{Results for the \textbf{analytic tumor\,/\,analytic velocity with non-zero diffusion (ATAV-DIF)} test case; ground truth: ($\rho_f=10$, $\rho_w=1$, $\rho_g=0$, $k_f=\num{1.0E-2}$, $k_w=1$, $k_g=0$, $\vect{p}=\vect{p}^\star$, $\vect{v}=-\vect{v}^\star$). We report values for the (summed) norm of the residual between the respective probability maps for the different brain tissue classes $\elltwoB$ and tumor $\elltwoT$ in patient space, the mean Dice coefficient for brain tissue $\diceB$ and tumor $\diceT$, respectively, as well as the relative norm of the gradient $\relG$ for the global coupled problem~\eqref{eq:global_opt}. We report results for different values of $\rho_f \in \{5,10,15\}$ used in the inversion ($\rho_f=10$ is the ground truth). We report the time spent per iteration (in seconds; top run) or in total (in seconds; bottom runs) for the entire Picard inversion, and the amount of that time spent in the tumor inversion and image registration (in percent (top run); in seconds (bottom runs)), respectively.  Note that the latter sums up to less than $100\%$ as we do not explicitly measure time spent in additional coupling functionality and forward solvers. These runs are performed using 64 MPI tasks on three nodes of \emph{HazelHen} (see \secref{s:hardware} for details). The top block shows the course of the inversion with respect to the Picard iteration index for the correct parameters (ground truth) for $\rho_f$ and $k_f$. The four rows on the bottom show the final result for our Picard scheme for different parameter and model combinations.}
\label{tab:ATAV-nonzero-diffusion}
\centering
\begin{small}
\begin{tabular}{crLlLlllll}
\toprule
iterations & $\beta_{\vect{v}}$ & $\elltwoB$         & $\diceB$           &  $\elltwoT$        & $\diceT$           & $\relG$            & $\rtIT$\,[s]       & $\rtTUM$\,[\%]      & $\rtREG$ [\%] \\
\midrule
\multicolumn{10}{l}{\emph{non-zero diffusion with ground truth parameters $\rho_f = 10, k_f=\num{1E-2}$}}\\
\midrule
ref  &  --           & \num{1.000000e+00} & \num{7.135000e-01} & \num{1.000000e+00} & \num{0.000000e+00} & \num{1.000000e+00} &  \\
$1$  &  \num{1e+00}  & \num{9.320000e-01} & \num{7.316000e-01} & \num{1.000000e+00} & \num{0.000000e+00} & \num{9.943000e-01} & \num{2.112000e+03} & \pernum{99.668561}  & \pernum{0.164962}  \\
$2$  &  \num{1e-01}  & \num{6.515000e-01} & \num{8.005000e-01} & \num{2.082000e-01} & \num{8.558000e-01} & \num{7.454000e-02} & \num{2.884000e+02} & \pernum{96.012483}  & \pernum{2.144938}  \\
$3$  &  \num{1e-02}  & \num{3.794000e-01} & \num{8.875000e-01} & \num{1.473000e-01} & \num{9.116000e-01} & \num{3.869000e-02} & \num{3.943000e+02} & \pernum{91.808268}  & \pernum{6.913518}  \\
$4$  &  \num{1e-03}  & \num{1.745000e-01} & \num{9.394000e-01} & \num{8.080000e-02} & \num{9.629000e-01} & \num{2.454000e-02} & \num{3.980000e+02} & \pernum{72.663317}  & \pernum{26.080402} \\
$5$  &  \num{1e-04}  & \num{1.601000e-01} & \num{9.475000e-01} & \num{5.929000e-02} & \num{9.781000e-01} & \num{1.770000e-02} & \num{2.003000e+02} & \pernum{35.411882}  & \pernum{62.106840} \\
$6$  &  \num{1e-04}  & \num{1.600000e-01} & \num{9.475000e-01} & \num{5.772000e-02} & \num{9.769000e-01} & \num{1.720000e-02} & \num{1.335000e+02} & \pernum{46.561798}  & \pernum{49.580524} \\
$7$  &  \num{1e-04}  & \num{1.599000e-01} & \num{9.474000e-01} & \num{5.627000e-02} & \num{9.758000e-01} & \num{1.733000e-02} & \num{7.099000e+01} & \pernum{0.0000000}  & \pernum{92.999014} \\
\midrule
\multicolumn{7}{l}{\emph{rvarying $\rho_f \in \{5,\boldsymbol{10},15\}, k_f=\num{1E-2}$, ground truth $\rho_f = 10, k_f=\num{1E-2}$}} & $\rtTOT$\,[s]       & $\rtTUM$\,[s]      & $\rtREG$ [s] \\
\midrule
$\rho_f = 5\phantom{0}$ &  \num{1e-04}  & \num{1.610000e-01}  & \num{9.462000e-01}  & \num{6.484000e-02}  & \num{9.674000e-01}  & \num{2.207000e-02}  & \num{4.374850e+03}  & \num{3.947620e+03}  & \num{3.967840e+02} \\
\highlightrow
$\rho_f = 10$ &  \num{1e-04}  & \num[math-rm=\mathbf]{1.599000e-01}  & \num[math-rm=\mathbf]{9.474000e-01}  & \num[math-rm=\mathbf]{5.627000e-02}  & \num[math-rm=\mathbf]{9.758000e-01}  & \num{1.733000e-02}  & \num{3.597490e+03}  & \num{3.166190e+03}  & \num{4.008240e+02} \\
$\rho_f = 15$ &  \num{1e-04}  & \num{1.613000e-01}  & \num{9.477000e-01}  & \num{6.393000e-02}  & \num{9.723000e-01}  & \num{1.411000e-02}  & \num{3.957320e+03}  & \num{3.527350e+03}  & \num{4.004410e+02} \\
\midrule
\multicolumn{7}{l}{\emph{$\rho_f 10, k_f=0$, ground truth $\rho_f = 10, k_f=\num{1E-2}$}} & $\rtTOT$\,[s]       & $\rtTUM$\,[s]      & $\rtREG$ [s] \\
\midrule
$\rho_f = 10$ &  \num{1e-04}  & \num{1.602000e-01}  & \num{9.477000e-01}  & \num{5.951000e-02}  & \num{9.711000e-01}  & \num{1.742000e-02}  & \num{4.252200e+02}  & \num{2.253460e+01}  & \num{4.009880e+02} \\
\bottomrule
\end{tabular}
\end{small}
\end{table*}

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Observations:} 
The most important observations are that \bipa\item the diffusion model does not have a significant impact on the quality of the inversion (Dice and mismatch) and that 
\item we are able to identify the correct growth rate used to construct the synthetic test problem\eipa.

In our formulation, we invert for the initial condition.\footnote{We can also invert for either the diffusion coefficient or the growth rate, see~\citep{Gholami:2016a}.}. This requires us to fix the growth rate as well as the diffusion coefficient. We can see that we obtain a slightly better mismatch (\num{5.627000e-02}) and Dice coefficient (\num{9.758000e-01}) for the tumor probability map if we use the correct $\rho_f$. These results suggest that we can identify the correct $\rho_f$ if we run multiple inversions for the initial condition. However, we note that these differences are small (the mismatch is between \num{5.951000e-02} and \num{5.627000e-02} and the Dice is between \num{9.711000e-01} and \num{9.758000e-01}, respectively, for the tumor). Overall, we obtain an excellent agreement between patient data and atlas data irrespective of the model choice. These observations are confirmed by careful visual inspection of \figref{fig:ATAV-nonzero-diffusion} (supplementary material; shows only results for the `'correct`' tumor parameters).

Note that we do not observe a significant deterioration if we switch off the diffusion operator (bottom line in \tabref{tab:ATAV-nonzero-diffusion}). This suggests that the diffusion operator plays a less critical role in our formulation. This can be explained by the parameterization of the initial condition. We can reconstruct complex tumor shapes even with a simple model. Overall, this indicates that using a reaction-only model might be sufficient for diffeomorphic image registration.\footnote{This is clearly not the case when targeting the design of computational framework to aid clinical  decision making by generating model based prediction of a patient's future tumor state. In this case, we quite certainly have to use more complex, high-fidelity models. We discuss this in more detail in \secref{s:conclusion}.} This is an important observation, since including the diffusion model is costly; the runtimes increase due to the higher costs in the tumor components. In particular, we observe an increase in runtime by a factor of 10 (compare the total run time for the last row in \tabref{tab:ATAV-nonzero-diffusion} to the total runtimes attained when enabling diffusion). If we switch off the diffusion, we can see that most work is done in the registration (for this experiment, the registration is about 20 times more expensive than the tumor component in our Picard scheme). However, if we enable the diffusion operator, the tumor inversion is about 10 times more expensive than the registration within our Picard scheme. Another interesting behavior within our scheme is that, during the first few iterations, most time is spent in the tumor inversion, whereas, as we reduce $\beta_{\vect{v}}$, the registration does most of the work. This is to be expected, since the runtime of our scheme (more precisely, the condition number of the Hessian) for diffeomorphic registration, is not independent of $\beta_{\vect{v}}$~\citep{Mang:2015a,Mang:2017a}; .

We can also observe that changes in the tumor model do not have a significant impact on the registration quality of the healthy part of the brain. The differences in the Dice coefficient and the residual are $\mathcal{O}(\num{1E-3})$.

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Conclusion:} The integration of a diffusion model into our inversion is very costly, at least for our current implementation. Designing a more efficient forward solver for the diffusion operator requires more work. We could demonstrate that our parameterization of the initial condition allows us to generate high-fidelity registration results, especially for the healthy anatomy, irrespective of the model that has been used to generate the data. These are clearly preliminary results, but they provide some evidence that reaction-only models might be sufficient for pure image registration (something that is quite certainly not the case if we target parameter identification and tumor growth prediction)~\citep{Hogea:2008a}. We further explore this hypothesis in the next experiment.

We can also observe that there are subtle differences in the reconstruction quality of the tumor if we use the `'correct`' growth rate for the inversion. Overall, we conclude that we can \bipa\item neglect the diffusion model in the context of diffeomorphic registration and \item might be able to identify appropriate growth rates if we run multiple inversions for different parameters\eipa.


==> 05-03-results_ATAV-LD.tex <==
%///////////////////////////////////////////////////////////////////////////////
\ipoint{Purpose:} We restruct the admissible initial condition parametrization for tumor growth to a very low dimensionality in order to exclude fully grown tumors as initial conditions. We examine, whether this increases the sensitivity of the reconstruction quality for the tumor with
respect to correct model parameters.

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Setup:} We use the same setting as in the former two experiments (ATAV-REAC and ATAV-DIF). The key difference here is that we enforce the initial tumor to be small, i.e., only invert for $n_{\vect{p}} = 8$ parameters, which results in a grid of $2 \times 2 \times 2$ Gaussians that cover the (in the ATAV cases known) true initial condition of the artificially grown tumor. We expect this to increase the sensitivity of our inversion with respect to the tumor parameters (we can not fully represent the whole patient tumor purely based on a linear combination of the basis functions).

Likewise to the ATAV-DIF test problem, we grow the artificial tumor using the full reaction-diffusion model (i.e., with diffusion and reaction enabled). The ground truth parameter used in the forward simulation to generate the synthetic test case are $\rho_f=15, \rho_w=1, \rho_g=0$ and $k_f=\num{1E-1}, k_w=1, k_g=0$. For the inversion, we again consider a variety of models and model parameter combinations, which includes the use of the `'correct`' (ground truth) tumor parameters. We also consider the case in which we completely neglect the tumor model (i.e., $\rho_f = k_f=0$) and just invert for the basis.

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Results:} We show simulation results in~\figref{fig:ATAV-nonzero-diffusion-sparse-ax-only} (for sagittal and coronal slices, \figref{fig:ATAV-nonzero-diffusion-sparse}) and report quantitative results in \tabref{tab:mismatch_ATAV-sparsity-of-initial-condition_non-zero-diffusion}. We plot the trend of the relative tumor mismatch with respect to the regularization parameter $\beta_{\vect{v}}$ for the Sobolev norm for the registration velocity (and by that the Picard iteration index) in \figref{fig:ATAV-SPARSE-MM-curves}.

%///////////////////////////////////////////////////////////////////////////////
\begin{figure}[h!]
\centering
\includegraphics[width=0.48\textwidth]{figures/TC1-ATAV-SPARSE/rel_tu-miss_over_betav_closeup.pdf}
\caption{\label{fig:ATAV-SPARSE-MM-curves}Mismatch reduction as a function of the regularization parameter $\beta_{\vect{v}}$ for the \textbf{analytic tumor with analytic velocity, diffusion and low-dimensional initial condition (ATAV-LD)} test case; ground truth: ($\rho_f=15$, $\rho_w=1$, $\rho_g=0$, $k_f=\num{1.0E-1}$, $k_w=1$, $k_g=0$, $\vect{p}=\vect{p}^\star$ (in patient domain), $\vect{v}$ N/A). We use an initial condition parameterized with only $n_{\vect{p}}=8$ Gaussians ($\sigma=\nicefrac{\pi}{15}$) and an analytic tumor with non-zero diffusion. The plot shows the relative mismatch for the tumor probability map $\elltwoT$ in patient space. Note that we reduce $\beta_{\vect{v}}$ by a factor of ten in each Picard iteration; the plot shows the mismatch reduction over the Picard iterations if read from right to left.}
\end{figure}

%///////////////////////////////////////////////////////////////////////////////
\begin{figure}[ht!]
\centering
\includegraphics[width=0.85\textwidth]{figures/TC1-ATAV-SPARSE/vis-ax-multiple-cases.pdf}
\caption{Tumor and brain labels for the \textbf{analythic tumor with analythic velocity with non-zero diffusion and low-dimensional initial condition (ATAV-LD)}
test case; ground truth: ($\rho_f=15$, $\rho_w=1$, $\rho_g=0$, $k_f=\num{1.0E-1}$, $k_w=1$, $k_g=0$, $\vect{p}=\vect{p}^\star$ (in patient domain), $\vect{v}$ N/A); for the 'correct' tumor parameters $\rho_f=15$, $k_f=\num{1.0E-1}$, and the two different settings $\rho_f=15$, $k_f=\num{5.0E-1}$ and $\rho_f=k_f=0$.}
\label{fig:ATAV-nonzero-diffusion-sparse-ax-only}
\end{figure}

%///////////////////////////////////////////////////////////////////////////////
\begin{table*}
\caption{Results for the \textbf{analytic tumor with analytic velocity with diffusion and low-dimensional initial condition (ATAV-LD)} test case;  ground truth: ($\rho_f=15$, $\rho_w=1$, $\rho_g=0$, $k_f=\num{1.0E-1}$, $k_w=1$, $k_g=0$, $\vect{p}=\vect{p}^\star$ (in patient domain), $\vect{v}$ N/A). We use a low-dimensional parameterization for the initial condition with $n_{\vect{p}}=8$ Gaussians ($\sigma=\nicefrac{\pi}{15}$). We report the (summed) mismatch for the probability maps for the brain tissue $\elltwoB$ and tumor $\elltwoT$ in patient space, the mean Dice coefficient for hard segmentations of brain tissue ($\diceB$) and tumor ($\diceT$), respectively, and the relative norm of the gradient ($\relG$) for the coupled problem \eqref{eq:global_opt}. We assess the final state of the reconstruction using different values for $\rho_f \in \{5,10,15, 20\}$ and $k_f \in \{0, \num{1E-1}\}$. Absolute timings are given for the tumor inversion and image registration, respectively using 64 MPI tasks on three nodes of HazelHen (see \secref{s:hardware} for details).  Note that the latter sums up to less than the reported total run time as we do not explicitly measure time spent in additional coupling functionality and forward solvers. We always reach the target value of $\beta_{\vect{v}} = \num{1E-4}$.}
\label{tab:mismatch_ATAV-sparsity-of-initial-condition_non-zero-diffusion}
\centering
\begin{small}
\begin{tabular}{llrrLlLlllll}
\toprule
$\rho$ & $k$  & It      & $\elltwoB$ & $\diceB$ & $  $\elltwoT$ $ & $\diceT$ & $\relG$  & $\rtTOT$\,[s] & $\rtTUM$\,[s] & $\rtREG$\,[s] \\
\midrule
     &            & initial & \num{1.000000e+00} & \num{7.176000e-01} & \num{1.000000e+00} & \num{0.000000e+00} & \num{1.000000e+00} & -- & -- & -- \\
\midrule
 $0$ & $0$          & final & \num{1.961000e-01} & \num{9.448000e-01} & \num{2.795000e-01} & \num{8.477000e-01} & \num{4.157000e-02} & \num{3.776320e+02} & \num{3.330000e+00} & \num{3.768990e+02} \\
$15$ & $0$          &       & \num{1.865000e-01} & \num{9.461000e-01} & \num{2.036000e-01} & \num{9.157000e-01} & \num{1.702000e-02} & \num{3.776650e+02} & \num{2.189700e+00} & \num{3.780200e+02} \\
\highlightrow
$15$ & $\num{1E-1}$ &       & \num[math-rm=\mathbf]{1.693000e-01} & \num[math-rm=\mathbf]{9.477000e-01} & \num[math-rm=\mathbf]{4.675000e-02} & \num[math-rm=\mathbf]{9.649000e-01} & \num{1.731000e-02} & \num{4.724960e+03} & \num{4.171100e+03} & \num{4.593420e+02} \\
$15$ & $\num{5E-1}$ &       & \num{1.901000e-01} & \num{9.412000e-01} & \num{3.365000e-01} & \num{4.714000e-02} & \num{1.782000e-02} & \num{6.670500e+03} & \num{5.538300e+03} & \num{4.289570e+02} \\
$15$ & $\num{1E-2}$ &       & \num{1.789000e-01} & \num{9.467000e-01} & \num{1.572000e-01} & \num{9.313000e-01} & \num{1.507000e-02} & \num{2.233390e+03} & \num{1.504600e+03} & \num{4.309730e+02} \\
 $5$ & $\num{1E-1}$ &       & \num{1.706000e-01} & \num{9.462000e-01} & \num{6.502000e-02} & \num{9.567000e-01} & \num{2.451000e-02} & \num{1.959840e+03} & \num{1.504300e+03} & \num{3.870510e+02} \\
$10$ & $\num{1E-1}$ &       & \num{1.695000e-01} & \num{9.467000e-01} & \num{4.976000e-02} & \num{9.620000e-01} & \num{2.006000e-02} & \num{3.900050e+03} & \num{2.902200e+03} & \num{3.725620e+02} \\
$10$ & $\num{1E-2}$ &       & \num{1.794000e-01} & \num{9.465000e-01} & \num{1.647000e-01} & \num{9.257000e-01} & \num{1.910000e-02} & \num{2.174100e+03} & \num{1.625260e+03} & \num{3.655810e+02} \\
$20$ & $\num{1E-1}$ &       & \num{1.695000e-01} & \num{9.477000e-01} & \num{5.445000e-02} & \num{9.559000e-01} & \num{2.018000e-02} & \num{3.073610e+03} & \num{2.617200e+03} & \num{3.881380e+02} \\
$20$ & $\num{1E-2}$ &       & \num{1.797000e-01} & \num{9.467000e-01} & \num{1.603000e-01} & \num{9.184000e-01} & \num{1.197000e-02} & \num{2.032620e+03} & \num{4.514000e+02} & \num{3.781680e+02} \\
\bottomrule
\end{tabular}
\end{small}
\end{table*}

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Observations:} The most important observation is that we can identify the correct pair of diffusion and reaction rate that has been used to generate the synthetic test case. Overall, we observe slightly more pronounced effects on the overall mismatch and Dice scores for the anatomy and, in particular, for the tumor if we do not use the ground truth parameters for the reaction and diffusion coefficients in our inversion as compared to our former experiment (in which we used a larger number of tumor initial condition parameters).

The sensitivity with respect to changes in the diffusion parameter $k_f$ is larger than with respect to changes in the growth rate $\rho_f$. We expect this much more pronounced dependence on the diffusion model if we parameterize the initial condition on a grid with a smaller support, since we need the cancerous cells to diffuse to areas more distant to the tumor center in order to be able to reconstruct the whole tumor. The trend of the relative mismatch for the tumor in \figref{fig:ATAV-SPARSE-MM-curves} highlights this effect. The curves almost cluster in terms of the different choices for the diffusion coefficient; we overall achieve significantly better mismatch if we choose the correct diffusion coefficient. We can also see that the curves plateau much earlier in cases where we use the wrong parameter combinations. The tumor mismatch takes values between \num{3.365000e-01} and \num{4.675000e-02} with a Dice score of \num{4.714000e-02} to \num{9.649000e-01}.

Overall, we again achieve an excellent mismatch for the anatomy, almost irrespective of the choices for the tumor model. The residual for the anatomy ranges from \num{1.693000e-01} to \num{1.901000e-01} and the Dice coefficient of \num{9.412000e-01} to \num{9.477000e-01}, respectively (the original Dice coefficient is \num{7.176000e-01}).

\ipoint{Conclusions:} If we do not use a large number of basis functions with a support that covers the entire patient's tumor, the choice of the correct set of parameters becomes more critical. We can observe that the inversion becomes more sensitive to perturbations in the tumor model parameters. We can either use a richer model with fewer parameters to represent the initial condition or increase the parameter space (i.e., $n_{\vect{p}}$) and by that the support for the grid of Gaussians to generate high-fidelity tumor reconstructions. Since the focus of this paper is image registration, and a richer model (diffusion) results in a significant increase in computational complexity and runtime (see \tabref{tab:ATAV-nonzero-diffusion} and \tabref{tab:mismatch_ATAV-sparsity-of-initial-condition_non-zero-diffusion}), we opt for an increased number of basis functions. This changes if our task is to provide predictive tumor growth tools where the identification of the correct
model ans its parameters is crucial. In this case, low-dimensional initial condition parametrizations are the better choice.

\FloatBarrier


==> 05-04-results_ATRV.tex <==
%%%%%%%%%%% TC semi-syn-tc-based-on-realdata (grown tumor in patient space)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%///////////////////////////////////////////////////////////////////////////////
\ipoint{Purpose:} We test our algorithm in the context of multi-subject registration for real brain data of two different individuals.

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Setup:} The patient data is no longer generated from the atlas image. We use an image of a different individual instead. Accordingly, we no longer know the ground truth velocity field. We grow an artificial tumor in a segmented, real patient brain.
%
%The atlas and the patient brain are taken from the \verb!689_templates!\AM{Name might have to be fixed}.
We solve the problem on a grid of size $N_i=256$, $i=0,1,2$. We choose $\vect{p}=\vect{p}^\star$ as an initial condition in the patient brain. The forward simulated tumor defines the template tumor $c_T$. We use the tumor parameters for the inversion that have been used for the generation of the synthetic test case. This test case is more challenging than ATAV since there is no `'ground truth`' for the tumor initial conditions in the atlas brain and for the registration velocity.

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Results:} We show simulation results and report quantitative results in~\figref{fig:mismatch_semi-syn-tc-nx-256}.

%///////////////////////////////////////////////////////////////////////////////
\begin{figure*}
\includegraphics[scale=.97]{figures/TC2-ATRV/{vis-all-labels-short-plain_ATRV-syn-tc}.pdf} \\
\centering
\begin{small}
\begin{tabular}{rrLlLlllll}
\toprule
iterations & $\beta_{\vect{v}}$ & $\elltwoB$ & $\diceB$ & $\elltwoT$ & $\diceT$ & $\relG$  & $\rtIT$\,[s] & $\rtTUM$\,[\%] & $\rtREG$\,[\%] \\
\midrule
initial &  --  & \num{1.000000e+00} & \num{6.559000e-01} & \num{1.000000e+00} & \num{0.000000e+00} & \num{1.000000e+00}  & -- & -- & -- \\
$  1$ &  \num{1e+00} & \num{9.354000e-01} & \num{6.867000e-01} & \num{1.000000e+00} & \num{0.000000e+00} & \num{9.980000e-01} & \num{6.031000e+01} & \pernum{46.327309} & \pernum{47.255845}  \\
$  2$ &  \num{1e-01} & \num{7.117000e-01} & \num{7.781000e-01} & \num{2.475000e-01} & \num{8.534000e-01} & \num{8.466000e-02} & \num{5.934000e+01} & \pernum{ 6.833502} & \pernum{92.467139}  \\
$  3$ &  \num{1e-02} & \num{4.477000e-01} & \num{8.769000e-01} & \num{1.904000e-01} & \num{9.107000e-01} & \num{3.331000e-02} & \num{1.514000e+03} & \pernum{ 0.251651} & \pernum{99.735799}  \\
$  4$ &  \num{1e-03} & \num{2.962000e-01} & \num{9.250000e-01} & \num{1.535000e-01} & \num{9.394000e-01} & \num{1.356000e-02} & \num{1.922000e+03} & \pernum{ 0.131686} & \pernum{99.843913}  \\
$  5$ &  \num{1e-04} & \num{2.663000e-01} & \num{9.335000e-01} & \num{1.450000e-01} & \num{9.475000e-01} & \num{1.023000e-02} & \num{4.309000e+02} & \pernum{ 0.331167} & \pernum{99.582270}  \\
$  6$ &  \num{1e-04} & \num{2.663000e-01} & \num{9.336000e-01} & \num{1.438000e-01} & \num{9.468000e-01} & \num{1.268000e-02} & \num{1.549000e+02} & \pernum{ 0.841188} & \pernum{98.902518}  \\
$  7$ &  \num{1e-04} & \num{2.662000e-01} & \num{9.336000e-01} & \num{1.431000e-01} & \num{9.462000e-01} & \num{1.238000e-02} & \num{1.513000e+02} & --                 & \pernum{99.735625}  \\
\midrule
final &  \num{1e-04} & \num{2.662000e-01} & \num{9.336000e-01} & \num{1.431000e-01} & \num{9.462000e-01} & \num{1.238000e-02} & \num{4.292750e+03} & \num{4.106600e+01}  & \num{4.274070e+03} \\
\bottomrule
\end{tabular}
\end{small}
\caption{Results for the \textbf{analytic tumor with real velocity (ATRV)} test case, ground truth:  ($\rho_f=15$, $\rho_w=1$, $\rho_g=0$, $k_f=0$, $\vect{p}=\vect{p}^\star$ (in patient domain); $\vect{v}$ N/A). The figure shows probability maps for the labels of the healthy atlas brain (top row) and the patient brain (with a synthetically generated tumor; bottom row). The patient's tumor is generated by solving the forward problem in the healthy patient dataset with an initial condition parameterized by $\vect{p}^\star$. We show axial slice $128$. We report the (summed) mismatch for the brain tissue probability maps ($\elltwoB$) and the tumor probability map ($\elltwoT$) in patient space, the mean Dice coefficient for the hard segmentation corresponding to the brain tissue ($\diceB$) and the tumor $\diceT$, respectively, as well as the relative norm of the gradient for the coupled problem \eqref{eq:global_opt} ($\relG$). We also show the run time per iteration in seconds ($\rtIT$), and the percentages ($\rtTUM$) and ($\rtREG$) of this runtime spent in the tumor solver and the image registration solver, respectively. Note that the latter sums up to less than $100\%$ as we do not explicitly measure time spent in additional coupling functionality and in the forward solvers. The last row shows the final values for mismatch and Dice as well as (accumulated) absolute run times for the sub-components in seconds.}\label{fig:mismatch_semi-syn-tc-nx-256}
\end{figure*}

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Observations} The most important observations are that \bipa\item we achieve an excellent registration quality with a Dice score of \num{9.336000e-01} and \num{9.462000e-01} for the hard segmentations for the anatomy and the tumor, respectively, and that \item our scheme seems to be still converging to a (local) minimizer of the join inversion-registration problem in this more realistic test case scenario\eipa.

Overall, the results slightly deteriorate as compared to the former test cases. We achieve a relative mismatch and Dice score for the anatomy that is about $\mathcal{O}(\num{1E-1})$ and $\mathcal{O}(\num{1E-2})$ worse, respectively, than in the former experiments. The reduction of the gradient of the coupled optimization problem of about two orders is comparable to the former test cases. Interestingly, there is a stronger imbalance between the time spent in the registration and the tumor inversion; the registration takes up more than 90\% of the runtime already in the second iteration. This indicates that running our solver on real inter-subject problems at a higher resolution significantly increases the complexity of the registration problem.

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Conclusion:} We conclude that we can still achieve an excellent registration quality with a Dice score of \num{9.336000e-01} and \num{9.462000e-01} for the hard segmentations for the anatomy and the tumor, respectively, if we perform our inversion on real brains of different individuals representing atlas and patient.


==> 05-05-results_ATRV-MF.tex <==
%%%%%%%%%%% TC semi-syn-tc-based-on-realdata, random tumor seed, multifocal (grown tumor in patient space)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%///////////////////////////////////////////////////////////////////////////////
\ipoint{Purpose:} We test the capabilities of our framework for the registration of an atlas to a patient's image that contains a multifocal tumor.

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Setup:} We use a similar setting as in the former section. The key difference is that our synthetically generated tumor is now a multifocal tumor, i.e., a tumor consisting of several separate components. The seeds $\vect{p}^\star$ for this tumor are chosen randomly. This in turn means that we have to choose the tumor growth initial condition parametrization adaptively in order to be able to recover all abnormal areas in the patient's image. This is an extremely important step to make our solver applicable to real patient data, something we will explore in the next section. The parametrization $\vect{p}=\vect{p}^\star$ for the growth of the artificial tumor in the patient brain is based on Gaussians arranged in a cube with center $(x^1,x^2,x^3) = 2\pi\cdot(0.5, 0.5, 0.5)$. The initial conditions are generated using random tumor seeds activating a maximum of $3$ Gaussians in the $x^3=\mbox{height}/2-$plane. This creates a multifocal template tumor $c_T$. We solve the forward problem with diffusion disabled, i.e., reaction-only. We employ the tumor parameters used to generate this artificial tumor also in our inversion.

Given that the tumor can now appear at two opposite locations in the brain (an interesting example for this is shown in \figref{fig:mismatch_ATRV-MF-fixed-semi-syn-nx-256}), we need to increase the support for the sub-domain that defines the grid of Gaussian basis functions. If we would just increase the size of this domain, we can no longer guarantee that the basis can represent complex initial conditions. We therefore use a larger number of parameters $n_{\vect{p}}$, namely 343 (see~\tabref{tab:tc-parameters}). The remaining parameters are set as defined in the setup of ARTV.

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Results:} We show simulation results and a summary of quantitative results for this test case in \figref{fig:mismatch_ATRV-MF-fixed-semi-syn-nx-256}.

%///////////////////////////////////////////////////////////////////////////////
\begin{figure*}
\centering
Run \#1 \hspace{5.8cm} Run \#2\\
\includegraphics[scale=.97]{figures/TC3-ATRV-MF/fixed/{vis-blended-its_2_ATRV-MF-syn-tc-1}.pdf}
\includegraphics[scale=.97]{figures/TC3-ATRV-MF/rand/{vis-blended-its_2_ATRV-MF-rand-syn-tc-2}.pdf}\\
\begin{small}
\begin{tabular}{rrrLlLlllll}
\toprule
\multicolumn{2}{l}{\textbf{run \#}}  & $\beta_{\vect{v}}$ & $\elltwoB$ & $\diceB$ & $\elltwoT$ & $\diceT$ & $\relG$  & $\rtTOT$\,[s] & $\rtTUM$\,[s] & $\rtREG$\,[s] \\
\midrule
%\multirow{ 2}{*}{\rotatebox{90}{\textit{RUN\,\#1}}} &
\multirow{ 2}{*}{$\runid$} &
initial &  --  & \num{1.000000e+00} & \num{6.452000e-01} & \num{1.000000e+00} & \num{0.000000e+00} & \num{1.000000e+00} &  -- & -- & -- \\
& final &  \num{1e-04}  & \num{2.643000e-01}  & \num{9.323000e-01}  & \num{1.425000e-01}  & \num{9.490000e-01}  & \num{1.752000e-02}  & \num{3.287310e+03}  & \num{3.087540e+02}  & \num{2.992270e+03} \\
\midrule
%\multirow{ 2}{*}{\rotatebox{90}{\textit{RUN\,\#2}}} &
\multirow{ 2}{*}{$\runid$} &
initial &  --  & \num{1.000000e+00} & \num{6.506000e-01} & \num{1.000000e+00} & \num{0.000000e+00} & \num{1.000000e+00} &  -- & -- & -- \\
& final &  \num{1e-04}  & \num{2.641000e-01}  & \num{9.298000e-01}  & \num{1.462000e-01}  & \num{9.518000e-01}  & \num{1.401000e-02}  & \num{4.912150e+03}  & \num{1.165800e+02}  & \num{4.811580e+03} \\
\bottomrule
\end{tabular}
\end{small}
\caption{Results for the \textbf{analytic multi-focal tumor with real velocity (ATRV-MF)} test case (two runs), ground truth: ($\rho_f=15$, $\rho_w=1$, $\rho_g=0$, $k_f=0$, $\vect{p}=\vect{p}^\star$ (in patient domain), $\vect{v}$ N/A). We display the healthy atlas brain ($k=1$), the reconstruction with tumor in patient space after the last Picard iteration ($k=7$), and the given segmented patient image with tumors (axial-slice 128; top block). We report the (summed) mismatch for the brain tissue probability maps ($\elltwoB$) and the tumor probability map ($\elltwoT$) in patient space, the mean Dice coefficient for the hard segmentation corresponding to the brain tissue ($\diceB$) and the tumor $\diceT$, respectively, as well as the relative norm of the gradient for the coupled problem \eqref{eq:global_opt} ($\relG$). We also show the run time until convergence of the Picard scheme in seconds ($\rtTOT$), and the (over all iterations accumulated) time ($\rtTUM$) and ($\rtREG$) spent in the tumor solver and the image registration solver, respectively. Note that the latter sums up to less than the reported total runtime as we do not explicitly measure time spent in additional coupling functionality as well as in the forward solvers.}
\label{fig:mismatch_ATRV-MF-fixed-semi-syn-nx-256}
\end{figure*}

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Observations}: The most important observation is that our adaptive parametrization and the Picard scheme is effective when it comes to the registration of a tumor-free atlas with a patient image that contains a multifocal tumor. We achieve almost the same Dice coefficient (up to between $\mathcal{O}(\num{1E-2})$ and $\mathcal{O}(\num{1E-3})$) for the hard segmentations associated with the probability maps for the tumor and brain anatomy, respectively. In particular, we can increase the Dice coefficient from \num{6.452000e-01} to \num{9.323000e-01} for run \#1 and from \num{6.506000e-01} to \num{9.298000e-01} for run \#2, respectively (see \figref{fig:mismatch_ATRV-MF-fixed-semi-syn-nx-256}). The Dice coefficient for the tumor is \num{9.490000e-01} and \num{9.518000e-01}, respectively. These values for the mismatch, Dice coefficient are comparable to what we achieved for ATRV. Moreover, we achieve a similar reduction of the relative norm of the coupled reduced gradient of about two orders of magnitude.

We can also see that the overall runtime for the tumor inversion increases as we increase the number of parameters, in particular from \num{4.106600e+01} seconds to \num{3.087540e+02} or \num{1.165800e+02} seconds, respectively (total tumor inversion runtimes in \figref{fig:mismatch_ATRV-MF-fixed-semi-syn-nx-256} and \figref{fig:mismatch_semi-syn-tc-nx-256}). However, this increase in runtime does not have a significant effect on the overall runtime of the total Picard scheme ($\mathcal{O}(\num{5E+3})$ seconds), which is dominated by the registration.

%///////////////////////////////////////////////////////////////////////////////
\ipoint{Conclusion:} We conclude from this part of the study that we can reconstruct multifocal tumors with the same quality and only slightly higher computational cost than for ATRV if we increase the number of Gaussian basis functions in the parametrization of the initial conditions.

